Interpretable Time Series Clustering Using Local Explanations

This study focuses on exploring the use of local interpretability methods for explaining time series clustering models. Many of the state-of-the-art clustering models are not directly explainable. To provide explanations for these clustering algorithms, we train classification models to estimate the cluster labels. Then, we use interpretability methods to explain the decisions of the classification models. The explanations are used to obtain insights into the clustering models. We perform a detailed numerical study to test the proposed approach on multiple datasets, clustering models, and classification models. The analysis of the results shows that the proposed approach can be used to explain time series clustering models, specifically when the underlying classification model is accurate. Lastly, we provide a detailed analysis of the results, discussing how our approach can be used in a real-life scenario.

==> old_tables_remove/classification_full.tex <==

\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{lllrrrrrr}
\rowcolor[HTML]{B0B3B2} 
\textbf{Dataset} & \textbf{Feature configuration} & \textbf{Model} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{\# Clusters}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{\begin{tabular}[c]{@{}l@{}}\# Clusters\\ post-processing\end{tabular}}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{F1 score}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Accuracy}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Precision}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Recall}} \\
Electricity      & with\_feats                    & XGB            & 10                                                               & 9                                                                                                                          & 0.890                                                         & 0.890                                                         & 0.895                                                          & 0.890                                                       \\
Electricity      & default                        & XGB            & 10                                                               & 9                                                                                                                          & 0.870                                                         & 0.870                                                         & 0.882                                                          & 0.870                                                       \\
Electricity      & with\_feats                    & KNN            & 10                                                               & 9                                                                                                                          & 0.859                                                         & 0.870                                                         & 0.878                                                          & 0.870                                                       \\
Electricity      & default                        & KNN            & 10                                                               & 9                                                                                                                          & 0.834                                                         & 0.860                                                         & 0.835                                                          & 0.860                                                       \\
Electricity      & default                        & FCN            & 10                                                               & 9                                                                                                                          & 0.779                                                         & 0.780                                                         & 0.820                                                          & 0.780                                                       \\
Electricity      & with\_feats                    & FCN            & 10                                                               & 9                                                                                                                          & 0.750                                                         & 0.750                                                         & 0.794                                                          & 0.750                                                       \\
Electricity      & feat\_only                     & XGB            & 10                                                               & 9                                                                                                                          & 0.639                                                         & 0.650                                                         & 0.649                                                          & 0.650                                                       \\
Electricity      & feat\_only                     & KNN            & 10                                                               & 9                                                                                                                          & 0.611                                                         & 0.640                                                         & 0.627                                                          & 0.640                                                       \\
Electricity      & feat\_only                     & FCN            & 10                                                               & 9                                                                                                                          & 0.580                                                         & 0.580                                                         & 0.592                                                          & 0.580                                                       \\
Electricity      & with\_feats                    & FCN            & 20                                                               & 15                                                                                                                         & 0.768                                                         & 0.788                                                         & 0.782                                                          & 0.788                                                       \\
Electricity      & default                        & KNN            & 20                                                               & 15                                                                                                                         & 0.758                                                         & 0.778                                                         & 0.796                                                          & 0.778                                                       \\
Electricity      & with\_feats                    & KNN            & 20                                                               & 15                                                                                                                         & 0.734                                                         & 0.747                                                         & 0.804                                                          & 0.747                                                       \\
Electricity      & default                        & FCN            & 20                                                               & 15                                                                                                                         & 0.724                                                         & 0.747                                                         & 0.776                                                          & 0.747                                                       \\
Electricity      & default                        & XGB            & 20                                                               & 15                                                                                                                         & 0.709                                                         & 0.727                                                         & 0.730                                                          & 0.727                                                       \\
Electricity      & with\_feats                    & XGB            & 20                                                               & 15                                                                                                                         & 0.615                                                         & 0.646                                                         & 0.636                                                          & 0.646                                                       \\
Electricity      & feat\_only                     & XGB            & 20                                                               & 15                                                                                                                         & 0.597                                                         & 0.616                                                         & 0.625                                                          & 0.616                                                       \\
Electricity      & feat\_only                     & FCN            & 20                                                               & 15                                                                                                                         & 0.547                                                         & 0.586                                                         & 0.561                                                          & 0.586                                                       \\
Electricity      & feat\_only                     & KNN            & 20                                                               & 15                                                                                                                         & 0.455                                                         & 0.505                                                         & 0.466                                                          & 0.505                                                       \\
Electricity      & default                        & KNN            & 40                                                               & 22                                                                                                                         & 0.718                                                         & 0.722                                                         & 0.781                                                          & 0.722                                                       \\
Electricity      & with\_feats                    & KNN            & 40                                                               & 22                                                                                                                         & 0.708                                                         & 0.722                                                         & 0.761                                                          & 0.722                                                       \\
Electricity      & with\_feats                    & FCN            & 40                                                               & 22                                                                                                                         & 0.611                                                         & 0.633                                                         & 0.646                                                          & 0.633                                                       \\
Electricity      & default                        & FCN            & 40                                                               & 22                                                                                                                         & 0.518                                                         & 0.556                                                         & 0.549                                                          & 0.556                                                       \\
Electricity      & with\_feats                    & XGB            & 40                                                               & 22                                                                                                                         & 0.432                                                         & 0.478                                                         & 0.427                                                          & 0.478                                                       \\
Electricity      & default                        & XGB            & 40                                                               & 22                                                                                                                         & 0.418                                                         & 0.467                                                         & 0.395                                                          & 0.467                                                       \\
Electricity      & feat\_only                     & XGB            & 40                                                               & 22                                                                                                                         & 0.414                                                         & 0.456                                                         & 0.398                                                          & 0.456                                                       \\
Electricity      & feat\_only                     & KNN            & 40                                                               & 22                                                                                                                         & 0.304                                                         & 0.344                                                         & 0.302                                                          & 0.344                                                       \\
Electricity      & feat\_only                     & FCN            & 40                                                               & 22                                                                                                                         & 0.292                                                         & 0.300                                                         & 0.322                                                          & 0.300                                                       \\
Pricing          & with\_feats                    & XGB            & 25                                                               & 16                                                                                                                         & 0.926                                                         & 0.927                                                         & 0.932                                                          & 0.927                                                       \\
Pricing          & with\_feats                    & FCN            & 25                                                               & 16                                                                                                                         & 0.919                                                         & 0.920                                                         & 0.920                                                          & 0.920                                                       \\
Pricing          & default                        & FCN            & 25                                                               & 16                                                                                                                         & 0.898                                                         & 0.903                                                         & 0.908                                                          & 0.903                                                       \\
Pricing          & default                        & XGB            & 25                                                               & 16                                                                                                                         & 0.897                                                         & 0.904                                                         & 0.896                                                          & 0.904                                                       \\
Pricing          & with\_feats                    & KNN            & 25                                                               & 16                                                                                                                         & 0.720                                                         & 0.755                                                         & 0.755                                                          & 0.755                                                       \\
Pricing          & default                        & KNN            & 25                                                               & 16                                                                                                                         & 0.699                                                         & 0.754                                                         & 0.707                                                          & 0.754                                                       \\
Pricing          & feat\_only                     & FCN            & 25                                                               & 16                                                                                                                         & 0.686                                                         & 0.700                                                         & 0.694                                                          & 0.700                                                       \\
Pricing          & feat\_only                     & XGB            & 25                                                               & 16                                                                                                                         & 0.684                                                         & 0.717                                                         & 0.688                                                          & 0.717                                                       \\
Pricing          & feat\_only                     & KNN            & 25                                                               & 16                                                                                                                         & 0.639                                                         & 0.673                                                         & 0.622                                                          & 0.673                                                       \\
Pricing          & with\_feats                    & XGB            & 50                                                               & 29                                                                                                                         & 0.894                                                         & 0.906                                                         & 0.893                                                          & 0.906                                                       \\
Pricing          & with\_feats                    & FCN            & 50                                                               & 29                                                                                                                         & 0.874                                                         & 0.880                                                         & 0.889                                                          & 0.880                                                       \\
Pricing          & default                        & XGB            & 50                                                               & 29                                                                                                                         & 0.873                                                         & 0.883                                                         & 0.876                                                          & 0.883                                                       \\
Pricing          & default                        & FCN            & 50                                                               & 29                                                                                                                         & 0.852                                                         & 0.857                                                         & 0.858                                                          & 0.857                                                       \\
Pricing          & with\_feats                    & KNN            & 50                                                               & 29                                                                                                                         & 0.701                                                         & 0.730                                                         & 0.698                                                          & 0.730                                                       \\
Pricing          & default                        & KNN            & 50                                                               & 29                                                                                                                         & 0.677                                                         & 0.697                                                         & 0.708                                                          & 0.697                                                       \\
Pricing          & feat\_only                     & XGB            & 50                                                               & 29                                                                                                                         & 0.673                                                         & 0.708                                                         & 0.709                                                          & 0.708                                                       \\
Pricing          & feat\_only                     & FCN            & 50                                                               & 29                                                                                                                         & 0.621                                                         & 0.643                                                         & 0.622                                                          & 0.643                                                       \\
Pricing          & feat\_only                     & KNN            & 50                                                               & 29                                                                                                                         & 0.556                                                         & 0.598                                                         & 0.544                                                          & 0.598                                                       \\
Pricing          & with\_feats                    & XGB            & 100                                                              & 43                                                                                                                         & 0.828                                                         & 0.842                                                         & 0.848                                                          & 0.842                                                       \\
Pricing          & default                        & XGB            & 100                                                              & 43                                                                                                                         & 0.821                                                         & 0.829                                                         & 0.834                                                          & 0.829                                                       \\
Pricing          & default                        & FCN            & 100                                                              & 43                                                                                                                         & 0.787                                                         & 0.793                                                         & 0.802                                                          & 0.793                                                       \\
Pricing          & with\_feats                    & FCN            & 100                                                              & 43                                                                                                                         & 0.752                                                         & 0.756                                                         & 0.763                                                          & 0.756                                                       \\
Pricing          & default                        & KNN            & 100                                                              & 43                                                                                                                         & 0.618                                                         & 0.652                                                         & 0.643                                                          & 0.652                                                       \\
Pricing          & feat\_only                     & XGB            & 100                                                              & 43                                                                                                                         & 0.606                                                         & 0.639                                                         & 0.614                                                          & 0.639                                                       \\
Pricing          & with\_feats                    & KNN            & 100                                                              & 43                                                                                                                         & 0.598                                                         & 0.625                                                         & 0.648                                                          & 0.625                                                       \\
Pricing          & feat\_only                     & FCN            & 100                                                              & 43                                                                                                                         & 0.565                                                         & 0.607                                                         & 0.564                                                          & 0.607                                                       \\
Pricing          & feat\_only                     & KNN            & 100                                                              & 43                                                                                                                         & 0.495                                                         & 0.526                                                         & 0.504                                                          & 0.526                                                       \\
Trace            & feat\_only                     & KNN            & 3                                                                & 3                                                                                                                          & 1.000                                                         & 1.000                                                         & 1.000                                                          & 1.000                                                       \\
Trace            & feat\_only                     & FCN            & 3                                                                & 3                                                                                                                          & 1.000                                                         & 1.000                                                         & 1.000                                                          & 1.000                                                       \\
Trace            & default                        & XGB            & 3                                                                & 3                                                                                                                          & 1.000                                                         & 1.000                                                         & 1.000                                                          & 1.000                                                       \\
Trace            & feat\_only                     & XGB            & 3                                                                & 3                                                                                                                          & 0.978                                                         & 0.978                                                         & 0.979                                                          & 0.978                                                       \\
Trace            & with\_feats                    & XGB            & 3                                                                & 3                                                                                                                          & 0.978                                                         & 0.978                                                         & 0.979                                                          & 0.978                                                       \\
Trace            & with\_feats                    & FCN            & 3                                                                & 3                                                                                                                          & 0.955                                                         & 0.956                                                         & 0.961                                                          & 0.956                                                       \\
Trace            & default                        & FCN            & 3                                                                & 3                                                                                                                          & 0.955                                                         & 0.956                                                         & 0.961                                                          & 0.956                                                       \\
Trace            & with\_feats                    & KNN            & 3                                                                & 3                                                                                                                          & 0.788                                                         & 0.800                                                         & 0.837                                                          & 0.800                                                       \\
Trace            & default                        & KNN            & 3                                                                & 3                                                                                                                          & 0.788                                                         & 0.800                                                         & 0.837                                                          & 0.800                                                       \\
Walmart          & with\_feats                    & XGB            & 10                                                               & 10                                                                                                                         & 0.905                                                         & 0.905                                                         & 0.906                                                          & 0.905                                                       \\
Walmart          & default                        & XGB            & 10                                                               & 10                                                                                                                         & 0.873                                                         & 0.872                                                         & 0.875                                                          & 0.872                                                       \\
Walmart          & default                        & KNN            & 10                                                               & 10                                                                                                                         & 0.856                                                         & 0.856                                                         & 0.864                                                          & 0.856                                                       \\
Walmart          & with\_feats                    & FCN            & 10                                                               & 10                                                                                                                         & 0.853                                                         & 0.853                                                         & 0.857                                                          & 0.853                                                       \\
Walmart          & with\_feats                    & KNN            & 10                                                               & 10                                                                                                                         & 0.846                                                         & 0.846                                                         & 0.849                                                          & 0.846                                                       \\
Walmart          & default                        & FCN            & 10                                                               & 10                                                                                                                         & 0.832                                                         & 0.831                                                         & 0.836                                                          & 0.831                                                       \\
Walmart          & feat\_only                     & XGB            & 10                                                               & 10                                                                                                                         & 0.797                                                         & 0.798                                                         & 0.798                                                          & 0.798                                                       \\
Walmart          & feat\_only                     & FCN            & 10                                                               & 10                                                                                                                         & 0.787                                                         & 0.788                                                         & 0.794                                                          & 0.788                                                       \\
Walmart          & feat\_only                     & KNN            & 10                                                               & 10                                                                                                                         & 0.716                                                         & 0.719                                                         & 0.719                                                          & 0.719                                                       \\
Walmart          & with\_feats                    & XGB            & 20                                                               & 20                                                                                                                         & 0.851                                                         & 0.852                                                         & 0.855                                                          & 0.852                                                       \\
Walmart          & default                        & XGB            & 20                                                               & 20                                                                                                                         & 0.850                                                         & 0.850                                                         & 0.853                                                          & 0.850                                                       \\
Walmart          & with\_feats                    & FCN            & 20                                                               & 20                                                                                                                         & 0.832                                                         & 0.833                                                         & 0.837                                                          & 0.833                                                       \\
Walmart          & default                        & FCN            & 20                                                               & 20                                                                                                                         & 0.823                                                         & 0.825                                                         & 0.826                                                          & 0.825                                                       \\
Walmart          & with\_feats                    & KNN            & 20                                                               & 20                                                                                                                         & 0.815                                                         & 0.817                                                         & 0.822                                                          & 0.817                                                       \\
Walmart          & default                        & KNN            & 20                                                               & 20                                                                                                                         & 0.802                                                         & 0.805                                                         & 0.808                                                          & 0.805                                                       \\
Walmart          & feat\_only                     & XGB            & 20                                                               & 20                                                                                                                         & 0.698                                                         & 0.703                                                         & 0.703                                                          & 0.703                                                       \\
Walmart          & feat\_only                     & FCN            & 20                                                               & 20                                                                                                                         & 0.680                                                         & 0.684                                                         & 0.703                                                          & 0.684                                                       \\
Walmart          & feat\_only                     & KNN            & 20                                                               & 20                                                                                                                         & 0.628                                                         & 0.637                                                         & 0.646                                                          & 0.637                                                       \\
Walmart          & with\_feats                    & XGB            & 40                                                               & 40                                                                                                                         & 0.796                                                         & 0.797                                                         & 0.809                                                          & 0.797                                                       \\
Walmart          & with\_feats                    & KNN            & 40                                                               & 40                                                                                                                         & 0.761                                                         & 0.768                                                         & 0.777                                                          & 0.768                                                       \\
Walmart          & default                        & KNN            & 40                                                               & 40                                                                                                                         & 0.759                                                         & 0.766                                                         & 0.778                                                          & 0.766                                                       \\
Walmart          & default                        & FCN            & 40                                                               & 40                                                                                                                         & 0.759                                                         & 0.762                                                         & 0.776                                                          & 0.762                                                       \\
Walmart          & with\_feats                    & FCN            & 40                                                               & 40                                                                                                                         & 0.729                                                         & 0.727                                                         & 0.757                                                          & 0.727                                                       \\
Walmart          & default                        & XGB            & 40                                                               & 40                                                                                                                         & 0.721                                                         & 0.723                                                         & 0.736                                                          & 0.723                                                       \\
Walmart          & feat\_only                     & XGB            & 40                                                               & 40                                                                                                                         & 0.606                                                         & 0.612                                                         & 0.616                                                          & 0.612                                                       \\
Walmart          & feat\_only                     & FCN            & 40                                                               & 40                                                                                                                         & 0.589                                                         & 0.607                                                         & 0.603                                                          & 0.607                                                       \\
Walmart          & feat\_only                     & KNN            & 40                                                               & 40                                                                                                                         & 0.477                                                         & 0.494                                                         & 0.486                                                          & 0.494                                                      
\end{tabular}
}

==> old_tables_remove/classification_seeds_full.tex <==
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{lllrrrrrrrrrr}
\rowcolor[HTML]{B0B3B2} 
\textbf{Dataset} & Feature configuration & \textbf{Model} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{\# Clusters}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{\begin{tabular}[c]{@{}l@{}}\# Clusters\\ post-processing\end{tabular}}} & \multicolumn{2}{l}{\cellcolor[HTML]{B0B3B2}\textbf{F1 score}} & \multicolumn{2}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Accuracy}} & \multicolumn{2}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Precision}} & \multicolumn{2}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Recall}} \\
                 &                       &                & \multicolumn{1}{l}{}                                             & \multicolumn{1}{l}{}                                                                                                       & \multicolumn{1}{l}{mean}       & \multicolumn{1}{l}{std}      & \multicolumn{1}{l}{mean}       & \multicolumn{1}{l}{std}      & \multicolumn{1}{l}{mean}       & \multicolumn{1}{l}{std}       & \multicolumn{1}{l}{mean}      & \multicolumn{1}{l}{std}     \\
Electricity      & with\_feats           & XGB            & 10                                                               & 9                                                                                                                          & 0.863                          & 0.013                        & 0.870                          & 0.007                        & 0.872                          & 0.026                         & 0.870                         & 0.007                       \\
Electricity      & default               & KNN          & 10                                                               & 9                                                                                                                          & 0.856                          & 0.030                        & 0.862                          & 0.029                        & 0.875                          & 0.027                         & 0.862                         & 0.029                       \\
Electricity      & default               & XGB            & 10                                                               & 9                                                                                                                          & 0.855                          & 0.033                        & 0.862                          & 0.025                        & 0.865                          & 0.041                         & 0.862                         & 0.025                       \\
Electricity      & with\_feats           & FCN            & 10                                                               & 9                                                                                                                          & 0.850                          & 0.030                        & 0.856                          & 0.025                        & 0.867                          & 0.025                         & 0.856                         & 0.025                       \\
Electricity      & with\_feats           & KNN          & 10                                                               & 9                                                                                                                          & 0.849                          & 0.043                        & 0.856                          & 0.039                        & 0.870                          & 0.037                         & 0.856                         & 0.039                       \\
Electricity      & default               & FCN            & 10                                                               & 9                                                                                                                          & 0.799                          & 0.058                        & 0.808                          & 0.048                        & 0.825                          & 0.044                         & 0.808                         & 0.048                       \\
Electricity      & feat\_only            & XGB            & 10                                                               & 9                                                                                                                          & 0.635                          & 0.039                        & 0.646                          & 0.036                        & 0.660                          & 0.033                         & 0.646                         & 0.036                       \\
Electricity      & feat\_only            & KNN          & 10                                                               & 9                                                                                                                          & 0.618                          & 0.032                        & 0.640                          & 0.037                        & 0.631                          & 0.041                         & 0.640                         & 0.037                       \\
Electricity      & feat\_only            & FCN            & 10                                                               & 9                                                                                                                          & 0.586                          & 0.045                        & 0.600                          & 0.040                        & 0.614                          & 0.025                         & 0.600                         & 0.040                       \\
Electricity      & default               & KNN          & 20                                                               & 15                                                                                                                         & 0.789                          & 0.031                        & 0.804                          & 0.030                        & 0.811                          & 0.029                         & 0.804                         & 0.030                       \\
Electricity      & with\_feats           & KNN          & 20                                                               & 15                                                                                                                         & 0.782                          & 0.024                        & 0.800                          & 0.022                        & 0.803                          & 0.022                         & 0.800                         & 0.022                       \\
Electricity      & with\_feats           & FCN            & 20                                                               & 15                                                                                                                         & 0.782                          & 0.015                        & 0.798                          & 0.016                        & 0.800                          & 0.015                         & 0.798                         & 0.016                       \\
Electricity      & default               & FCN            & 20                                                               & 15                                                                                                                         & 0.732                          & 0.051                        & 0.749                          & 0.051                        & 0.737                          & 0.054                         & 0.749                         & 0.051                       \\
Electricity      & with\_feats           & XGB            & 20                                                               & 15                                                                                                                         & 0.711                          & 0.036                        & 0.723                          & 0.040                        & 0.720                          & 0.036                         & 0.723                         & 0.040                       \\
Electricity      & default               & XGB            & 20                                                               & 15                                                                                                                         & 0.700                          & 0.020                        & 0.715                          & 0.021                        & 0.714                          & 0.027                         & 0.715                         & 0.021                       \\
Electricity      & feat\_only            & XGB            & 20                                                               & 15                                                                                                                         & 0.592                          & 0.012                        & 0.610                          & 0.006                        & 0.601                          & 0.020                         & 0.610                         & 0.006                       \\
Electricity      & feat\_only            & FCN            & 20                                                               & 15                                                                                                                         & 0.507                          & 0.016                        & 0.515                          & 0.024                        & 0.524                          & 0.021                         & 0.515                         & 0.024                       \\
Electricity      & feat\_only            & KNN          & 20                                                               & 15                                                                                                                         & 0.474                          & 0.032                        & 0.501                          & 0.035                        & 0.478                          & 0.029                         & 0.501                         & 0.035                       \\
Electricity      & default               & KNN          & 40                                                               & 22                                                                                                                         & 0.705                          & 0.043                        & 0.740                          & 0.042                        & 0.728                          & 0.026                         & 0.740                         & 0.042                       \\
Electricity      & with\_feats           & KNN          & 40                                                               & 22                                                                                                                         & 0.700                          & 0.031                        & 0.733                          & 0.028                        & 0.728                          & 0.033                         & 0.733                         & 0.028                       \\
Electricity      & with\_feats           & FCN            & 40                                                               & 22                                                                                                                         & 0.604                          & 0.033                        & 0.631                          & 0.024                        & 0.629                          & 0.041                         & 0.631                         & 0.024                       \\
Electricity      & default               & FCN            & 40                                                               & 22                                                                                                                         & 0.594                          & 0.087                        & 0.616                          & 0.088                        & 0.612                          & 0.071                         & 0.616                         & 0.088                       \\
Electricity      & with\_feats           & XGB            & 40                                                               & 22                                                                                                                         & 0.545                          & 0.065                        & 0.562                          & 0.061                        & 0.556                          & 0.072                         & 0.562                         & 0.061                       \\
Electricity      & default               & XGB            & 40                                                               & 22                                                                                                                         & 0.504                          & 0.085                        & 0.529                          & 0.084                        & 0.525                          & 0.087                         & 0.529                         & 0.084                       \\
Electricity      & feat\_only            & XGB            & 40                                                               & 22                                                                                                                         & 0.408                          & 0.027                        & 0.427                          & 0.037                        & 0.418                          & 0.036                         & 0.427                         & 0.037                       \\
Electricity      & feat\_only            & FCN            & 40                                                               & 22                                                                                                                         & 0.352                          & 0.032                        & 0.371                          & 0.030                        & 0.377                          & 0.026                         & 0.371                         & 0.030                       \\
Electricity      & feat\_only            & KNN          & 40                                                               & 22                                                                                                                         & 0.340                          & 0.021                        & 0.369                          & 0.014                        & 0.366                          & 0.042                         & 0.369                         & 0.014                       \\
Pricing          & default               & XGB            & 25                                                               & 16                                                                                                                         & 0.892                          & 0.008                        & 0.903                          & 0.008                        & 0.895                          & 0.009                         & 0.903                         & 0.008                       \\
Pricing          & with\_feats           & XGB            & 25                                                               & 16                                                                                                                         & 0.887                          & 0.020                        & 0.899                          & 0.015                        & 0.890                          & 0.023                         & 0.899                         & 0.015                       \\
Pricing          & with\_feats           & FCN            & 25                                                               & 16                                                                                                                         & 0.881                          & 0.010                        & 0.889                          & 0.009                        & 0.888                          & 0.011                         & 0.889                         & 0.009                       \\
Pricing          & default               & FCN            & 25                                                               & 16                                                                                                                         & 0.873                          & 0.015                        & 0.879                          & 0.018                        & 0.878                          & 0.012                         & 0.879                         & 0.018                       \\
Pricing          & feat\_only            & XGB            & 25                                                               & 16                                                                                                                         & 0.714                          & 0.030                        & 0.737                          & 0.028                        & 0.727                          & 0.039                         & 0.737                         & 0.028                       \\
Pricing          & with\_feats           & KNN          & 25                                                               & 16                                                                                                                         & 0.705                          & 0.010                        & 0.744                          & 0.009                        & 0.722                          & 0.009                         & 0.744                         & 0.009                       \\
Pricing          & default               & KNN          & 25                                                               & 16                                                                                                                         & 0.684                          & 0.026                        & 0.728                          & 0.025                        & 0.729                          & 0.025                         & 0.728                         & 0.025                       \\
Pricing          & feat\_only            & FCN            & 25                                                               & 16                                                                                                                         & 0.670                          & 0.025                        & 0.682                          & 0.025                        & 0.674                          & 0.030                         & 0.682                         & 0.025                       \\
Pricing          & feat\_only            & KNN          & 25                                                               & 16                                                                                                                         & 0.631                          & 0.029                        & 0.672                          & 0.029                        & 0.621                          & 0.030                         & 0.672                         & 0.029                       \\
Pricing          & with\_feats           & XGB            & 50                                                               & 29                                                                                                                         & 0.893                          & 0.007                        & 0.903                          & 0.005                        & 0.900                          & 0.006                         & 0.903                         & 0.005                       \\
Pricing          & with\_feats           & FCN            & 50                                                               & 29                                                                                                                         & 0.876                          & 0.010                        & 0.882                          & 0.011                        & 0.882                          & 0.007                         & 0.882                         & 0.011                       \\
Pricing          & default               & XGB            & 50                                                               & 29                                                                                                                         & 0.872                          & 0.029                        & 0.882                          & 0.027                        & 0.881                          & 0.026                         & 0.882                         & 0.027                       \\
Pricing          & default               & FCN            & 50                                                               & 29                                                                                                                         & 0.863                          & 0.016                        & 0.872                          & 0.014                        & 0.870                          & 0.017                         & 0.872                         & 0.014                       \\
Pricing          & default               & KNN          & 50                                                               & 29                                                                                                                         & 0.684                          & 0.030                        & 0.718                          & 0.028                        & 0.700                          & 0.031                         & 0.718                         & 0.028                       \\
Pricing          & with\_feats           & KNN          & 50                                                               & 29                                                                                                                         & 0.681                          & 0.022                        & 0.716                          & 0.020                        & 0.698                          & 0.021                         & 0.716                         & 0.020                       \\
Pricing          & feat\_only            & XGB            & 50                                                               & 29                                                                                                                         & 0.660                          & 0.032                        & 0.694                          & 0.031                        & 0.665                          & 0.030                         & 0.694                         & 0.031                       \\
Pricing          & feat\_only            & FCN            & 50                                                               & 29                                                                                                                         & 0.633                          & 0.021                        & 0.647                          & 0.020                        & 0.644                          & 0.026                         & 0.647                         & 0.020                       \\
Pricing          & feat\_only            & KNN          & 50                                                               & 29                                                                                                                         & 0.568                          & 0.017                        & 0.603                          & 0.022                        & 0.551                          & 0.013                         & 0.603                         & 0.022                       \\
Pricing          & default               & XGB            & 100                                                              & 43                                                                                                                         & 0.816                          & 0.028                        & 0.830                          & 0.026                        & 0.830                          & 0.026                         & 0.830                         & 0.026                       \\
Pricing          & with\_feats           & XGB            & 100                                                              & 43                                                                                                                         & 0.795                          & 0.013                        & 0.810                          & 0.009                        & 0.811                          & 0.015                         & 0.810                         & 0.009                       \\
Pricing          & with\_feats           & FCN            & 100                                                              & 43                                                                                                                         & 0.781                          & 0.019                        & 0.791                          & 0.018                        & 0.794                          & 0.024                         & 0.791                         & 0.018                       \\
Pricing          & default               & FCN            & 100                                                              & 43                                                                                                                         & 0.777                          & 0.035                        & 0.788                          & 0.033                        & 0.787                          & 0.032                         & 0.788                         & 0.033                       \\
Pricing          & with\_feats           & KNN          & 100                                                              & 43                                                                                                                         & 0.604                          & 0.018                        & 0.639                          & 0.016                        & 0.623                          & 0.027                         & 0.639                         & 0.016                       \\
Pricing          & default               & KNN          & 100                                                              & 43                                                                                                                         & 0.599                          & 0.017                        & 0.630                          & 0.012                        & 0.634                          & 0.027                         & 0.630                         & 0.012                       \\
Pricing          & feat\_only            & XGB            & 100                                                              & 43                                                                                                                         & 0.566                          & 0.016                        & 0.601                          & 0.015                        & 0.582                          & 0.020                         & 0.601                         & 0.015                       \\
Pricing          & feat\_only            & FCN            & 100                                                              & 43                                                                                                                         & 0.559                          & 0.023                        & 0.569                          & 0.031                        & 0.578                          & 0.031                         & 0.569                         & 0.031                       \\
Pricing          & feat\_only            & KNN          & 100                                                              & 43                                                                                                                         & 0.482                          & 0.020                        & 0.516                          & 0.021                        & 0.478                          & 0.017                         & 0.516                         & 0.021                       \\
Trace            & feat\_only            & FCN            & 3                                                                & 3                                                                                                                          & 1.000                          & 0.000                        & 1.000                          & 0.000                        & 1.000                          & 0.000                         & 1.000                         & 0.000                       \\
Trace            & feat\_only            & KNN          & 3                                                                & 3                                                                                                                          & 1.000                          & 0.000                        & 1.000                          & 0.000                        & 1.000                          & 0.000                         & 1.000                         & 0.000                       \\
Trace            & feat\_only            & XGB            & 3                                                                & 3                                                                                                                          & 1.000                          & 0.000                        & 1.000                          & 0.000                        & 1.000                          & 0.000                         & 1.000                         & 0.000                       \\
Trace            & with\_feats           & XGB            & 3                                                                & 3                                                                                                                          & 1.000                          & 0.000                        & 1.000                          & 0.000                        & 1.000                          & 0.000                         & 1.000                         & 0.000                       \\
Trace            & with\_feats           & FCN            & 3                                                                & 3                                                                                                                          & 0.996                          & 0.010                        & 0.996                          & 0.010                        & 0.996                          & 0.009                         & 0.996                         & 0.010                       \\
Trace            & with\_feats           & KNN          & 3                                                                & 3                                                                                                                          & 0.798                          & 0.044                        & 0.813                          & 0.037                        & 0.870                          & 0.037                         & 0.813                         & 0.037                       \\
Trace            & default               & XGB            & 3                                                                & 3                                                                                                                          & 0.312                          & 0.044                        & 0.316                          & 0.043                        & 0.317                          & 0.043                         & 0.316                         & 0.043                       \\
Trace            & default               & KNN          & 3                                                                & 3                                                                                                                          & 0.291                          & 0.070                        & 0.307                          & 0.064                        & 0.299                          & 0.063                         & 0.307                         & 0.064                       \\
Trace            & default               & FCN            & 3                                                                & 3                                                                                                                          & 0.247                          & 0.051                        & 0.271                          & 0.040                        & 0.266                          & 0.060                         & 0.271                         & 0.040                       \\
Walmart          & with\_feats           & XGB            & 10                                                               & 10                                                                                                                         & 0.895                          & 0.010                        & 0.895                          & 0.010                        & 0.897                          & 0.009                         & 0.895                         & 0.010                       \\
Walmart          & default               & XGB            & 10                                                               & 10                                                                                                                         & 0.871                          & 0.007                        & 0.870                          & 0.007                        & 0.875                          & 0.006                         & 0.870                         & 0.007                       \\
Walmart          & with\_feats           & FCN            & 10                                                               & 10                                                                                                                         & 0.866                          & 0.021                        & 0.866                          & 0.021                        & 0.873                          & 0.020                         & 0.866                         & 0.021                       \\
Walmart          & with\_feats           & KNN          & 10                                                               & 10                                                                                                                         & 0.838                          & 0.017                        & 0.839                          & 0.017                        & 0.843                          & 0.017                         & 0.839                         & 0.017                       \\
Walmart          & default               & KNN          & 10                                                               & 10                                                                                                                         & 0.838                          & 0.014                        & 0.838                          & 0.013                        & 0.843                          & 0.014                         & 0.838                         & 0.013                       \\
Walmart          & default               & FCN            & 10                                                               & 10                                                                                                                         & 0.838                          & 0.026                        & 0.839                          & 0.026                        & 0.845                          & 0.021                         & 0.839                         & 0.026                       \\
Walmart          & feat\_only            & XGB            & 10                                                               & 10                                                                                                                         & 0.797                          & 0.008                        & 0.799                          & 0.008                        & 0.802                          & 0.007                         & 0.799                         & 0.008                       \\
Walmart          & feat\_only            & FCN            & 10                                                               & 10                                                                                                                         & 0.777                          & 0.012                        & 0.781                          & 0.011                        & 0.784                          & 0.011                         & 0.781                         & 0.011                       \\
Walmart          & feat\_only            & KNN          & 10                                                               & 10                                                                                                                         & 0.725                          & 0.013                        & 0.728                          & 0.011                        & 0.731                          & 0.012                         & 0.728                         & 0.011                       \\
Walmart          & with\_feats           & XGB            & 20                                                               & 20                                                                                                                         & 0.856                          & 0.013                        & 0.856                          & 0.013                        & 0.860                          & 0.012                         & 0.856                         & 0.013                       \\
Walmart          & with\_feats           & FCN            & 20                                                               & 20                                                                                                                         & 0.829                          & 0.016                        & 0.830                          & 0.016                        & 0.840                          & 0.012                         & 0.830                         & 0.016                       \\
Walmart          & default               & XGB            & 20                                                               & 20                                                                                                                         & 0.828                          & 0.017                        & 0.828                          & 0.017                        & 0.834                          & 0.016                         & 0.828                         & 0.017                       \\
Walmart          & default               & FCN            & 20                                                               & 20                                                                                                                         & 0.811                          & 0.020                        & 0.812                          & 0.020                        & 0.822                          & 0.015                         & 0.812                         & 0.020                       \\
Walmart          & with\_feats           & KNN          & 20                                                               & 20                                                                                                                         & 0.809                          & 0.012                        & 0.811                          & 0.012                        & 0.816                          & 0.012                         & 0.811                         & 0.012                       \\
Walmart          & default               & KNN          & 20                                                               & 20                                                                                                                         & 0.806                          & 0.008                        & 0.808                          & 0.007                        & 0.813                          & 0.008                         & 0.808                         & 0.007                       \\
Walmart          & feat\_only            & XGB            & 20                                                               & 20                                                                                                                         & 0.699                          & 0.021                        & 0.705                          & 0.020                        & 0.701                          & 0.020                         & 0.705                         & 0.020                       \\
Walmart          & feat\_only            & FCN            & 20                                                               & 20                                                                                                                         & 0.674                          & 0.015                        & 0.686                          & 0.010                        & 0.690                          & 0.011                         & 0.686                         & 0.010                       \\
Walmart          & feat\_only            & KNN          & 20                                                               & 20                                                                                                                         & 0.616                          & 0.010                        & 0.626                          & 0.012                        & 0.633                          & 0.014                         & 0.626                         & 0.012                       \\
Walmart          & with\_feats           & XGB            & 40                                                               & 40                                                                                                                         & 0.784                          & 0.011                        & 0.785                          & 0.011                        & 0.796                          & 0.009                         & 0.785                         & 0.011                       \\
Walmart          & with\_feats           & KNN          & 40                                                               & 40                                                                                                                         & 0.773                          & 0.012                        & 0.777                          & 0.011                        & 0.785                          & 0.011                         & 0.777                         & 0.011                       \\
Walmart          & with\_feats           & FCN            & 40                                                               & 40                                                                                                                         & 0.768                          & 0.021                        & 0.772                          & 0.020                        & 0.785                          & 0.016                         & 0.772                         & 0.020                       \\
Walmart          & default               & KNN          & 40                                                               & 40                                                                                                                         & 0.767                          & 0.013                        & 0.772                          & 0.013                        & 0.779                          & 0.012                         & 0.772                         & 0.013                       \\
Walmart          & default               & FCN            & 40                                                               & 40                                                                                                                         & 0.758                          & 0.014                        & 0.763                          & 0.013                        & 0.773                          & 0.013                         & 0.763                         & 0.013                       \\
Walmart          & default               & XGB            & 40                                                               & 40                                                                                                                         & 0.729                          & 0.013                        & 0.730                          & 0.014                        & 0.743                          & 0.014                         & 0.730                         & 0.014                       \\
Walmart          & feat\_only            & XGB            & 40                                                               & 40                                                                                                                         & 0.585                          & 0.013                        & 0.590                          & 0.012                        & 0.596                          & 0.013                         & 0.590                         & 0.012                       \\
Walmart          & feat\_only            & FCN            & 40                                                               & 40                                                                                                                         & 0.566                          & 0.012                        & 0.582                          & 0.010                        & 0.595                          & 0.012                         & 0.582                         & 0.010                       \\
Walmart          & feat\_only            & KNN          & 40                                                               & 40                                                                                                                         & 0.491                          & 0.015                        & 0.504                          & 0.012                        & 0.516                          & 0.020                         & 0.504                         & 0.012                      
\end{tabular}
}

==> old_tables_remove/clustering_results.tex <==
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{lrrrrr}
\rowcolor[HTML]{B0B3B2} 
\textbf{Dataset}                & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{\# Clusters}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Silhouette Score}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Calinski-Harabasz Score}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Davies Bouldin Score}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Inertia}} \\
Electricity                     & 10                                                               & 0.144                                                                 & 59.64                                                                        & 1.733                                                                     & 1107                                                         \\
Electricity                     & 20                                                               & 0.104                                                                 & 40.42                                                                        & 1.524                                                                     & 854                                                          \\
Electricity                     & 30                                                               & 0.088                                                                 & 32.01                                                                        & 1.481                                                                     & 726                                                          \\
Electricity                     & 40                                                               & 0.075                                                                 & 26.84                                                                        & 1.537                                                                     & 646                                                          \\
Walmart                         & 10                                                               & 0.112                                                                 & 340.93                                                                       & 2.204                                                                     & 8096                                                         \\
Walmart                         & 20                                                               & 0.111                                                                 & 208.95                                                                       & 2.086                                                                     & 6978                                                         \\
Walmart                         & 30                                                               & 0.102                                                                 & 158.30                                                                       & 2.198                                                                     & 6364                                                         \\
Walmart                         & 40                                                               & 0.097                                                                 & 128.50                                                                       & 2.262                                                                     & 5998                                                         \\
Pricing                         & 25                                                               & -0.230                                                                & 3.65                                                                         & 3.104                                                                     & 6560                                                         \\
\cellcolor[HTML]{FFFFFF}Pricing & 50                                                               & -0.310                                                                & 3.79                                                                         & 2.692                                                                     & 6175                                                         \\
\cellcolor[HTML]{FFFFFF}Pricing & 75                                                               & -0.320                                                                & 3.43                                                                         & 2.542                                                                     & 5999                                                         \\
\cellcolor[HTML]{FFFFFF}Pricing & 100                                                              & -0.309                                                                & 3.27                                                                         & 2.424                                                                     & 5711                                                        
\end{tabular}
}

==> old_tables_remove/datasets.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
& \textbf{Pricing} & \textbf{Trace} & \textbf{Walmart} & \textbf{Electricity}\\ \hline
\# time series     & 1,160         & 200 & 2,660 & 370 \\ \hline
Domain             & $\mathbb{R}_+$ & $\mathbb{R}$ & $\mathbb{N}$ & $\mathbb{R}_+$ \\ \hline
% \# time covariates & 4           &  3  & 4   & 0 \\ \hline
\# timesteps & 571        &  275 & 143  & 168 \\ \hline
Time Granularity     & Daily      & Seconds & Weekly & Hourly \\ \hline
\end{tabular} % Can add num training examples

==> tables/R3/classification_full.tex <==

\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{lllrrrrrr}
\rowcolor[HTML]{B0B3B2} 
\textbf{Dataset} & \textbf{Feature configuration} & \textbf{Model} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{\# Clusters}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{\begin{tabular}[c]{@{}l@{}}\# Clusters\\ post-processing\end{tabular}}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{F1 score}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Accuracy}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Precision}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Recall}} \\
Electricity      & with\_feats                    & XGB            & 10                                                               & 9                                                                                                                          & 0.890                                                         & 0.890                                                         & 0.895                                                          & 0.890                                                       \\
Electricity      & default                        & XGB            & 10                                                               & 9                                                                                                                          & 0.870                                                         & 0.870                                                         & 0.882                                                          & 0.870                                                       \\
Electricity      & with\_feats                    & KNN            & 10                                                               & 9                                                                                                                          & 0.859                                                         & 0.870                                                         & 0.878                                                          & 0.870                                                       \\
Electricity      & default                        & KNN            & 10                                                               & 9                                                                                                                          & 0.834                                                         & 0.860                                                         & 0.835                                                          & 0.860                                                       \\
Electricity      & default                        & FCN            & 10                                                               & 9                                                                                                                          & 0.779                                                         & 0.780                                                         & 0.820                                                          & 0.780                                                       \\
Electricity      & with\_feats                    & FCN            & 10                                                               & 9                                                                                                                          & 0.750                                                         & 0.750                                                         & 0.794                                                          & 0.750                                                       \\
Electricity      & feat\_only                     & XGB            & 10                                                               & 9                                                                                                                          & 0.639                                                         & 0.650                                                         & 0.649                                                          & 0.650                                                       \\
Electricity      & feat\_only                     & KNN            & 10                                                               & 9                                                                                                                          & 0.611                                                         & 0.640                                                         & 0.627                                                          & 0.640                                                       \\
Electricity      & feat\_only                     & FCN            & 10                                                               & 9                                                                                                                          & 0.580                                                         & 0.580                                                         & 0.592                                                          & 0.580                                                       \\
Electricity      & with\_feats                    & FCN            & 20                                                               & 15                                                                                                                         & 0.768                                                         & 0.788                                                         & 0.782                                                          & 0.788                                                       \\
Electricity      & default                        & KNN            & 20                                                               & 15                                                                                                                         & 0.758                                                         & 0.778                                                         & 0.796                                                          & 0.778                                                       \\
Electricity      & with\_feats                    & KNN            & 20                                                               & 15                                                                                                                         & 0.734                                                         & 0.747                                                         & 0.804                                                          & 0.747                                                       \\
Electricity      & default                        & FCN            & 20                                                               & 15                                                                                                                         & 0.724                                                         & 0.747                                                         & 0.776                                                          & 0.747                                                       \\
Electricity      & default                        & XGB            & 20                                                               & 15                                                                                                                         & 0.709                                                         & 0.727                                                         & 0.730                                                          & 0.727                                                       \\
Electricity      & with\_feats                    & XGB            & 20                                                               & 15                                                                                                                         & 0.615                                                         & 0.646                                                         & 0.636                                                          & 0.646                                                       \\
Electricity      & feat\_only                     & XGB            & 20                                                               & 15                                                                                                                         & 0.597                                                         & 0.616                                                         & 0.625                                                          & 0.616                                                       \\
Electricity      & feat\_only                     & FCN            & 20                                                               & 15                                                                                                                         & 0.547                                                         & 0.586                                                         & 0.561                                                          & 0.586                                                       \\
Electricity      & feat\_only                     & KNN            & 20                                                               & 15                                                                                                                         & 0.455                                                         & 0.505                                                         & 0.466                                                          & 0.505                                                       \\
Electricity      & default                        & KNN            & 40                                                               & 22                                                                                                                         & 0.718                                                         & 0.722                                                         & 0.781                                                          & 0.722                                                       \\
Electricity      & with\_feats                    & KNN            & 40                                                               & 22                                                                                                                         & 0.708                                                         & 0.722                                                         & 0.761                                                          & 0.722                                                       \\
Electricity      & with\_feats                    & FCN            & 40                                                               & 22                                                                                                                         & 0.611                                                         & 0.633                                                         & 0.646                                                          & 0.633                                                       \\
Electricity      & default                        & FCN            & 40                                                               & 22                                                                                                                         & 0.518                                                         & 0.556                                                         & 0.549                                                          & 0.556                                                       \\
Electricity      & with\_feats                    & XGB            & 40                                                               & 22                                                                                                                         & 0.432                                                         & 0.478                                                         & 0.427                                                          & 0.478                                                       \\
Electricity      & default                        & XGB            & 40                                                               & 22                                                                                                                         & 0.418                                                         & 0.467                                                         & 0.395                                                          & 0.467                                                       \\
Electricity      & feat\_only                     & XGB            & 40                                                               & 22                                                                                                                         & 0.414                                                         & 0.456                                                         & 0.398                                                          & 0.456                                                       \\
Electricity      & feat\_only                     & KNN            & 40                                                               & 22                                                                                                                         & 0.304                                                         & 0.344                                                         & 0.302                                                          & 0.344                                                       \\
Electricity      & feat\_only                     & FCN            & 40                                                               & 22                                                                                                                         & 0.292                                                         & 0.300                                                         & 0.322                                                          & 0.300                                                       \\
Pricing          & with\_feats                    & XGB            & 25                                                               & 16                                                                                                                         & 0.926                                                         & 0.927                                                         & 0.932                                                          & 0.927                                                       \\
Pricing          & with\_feats                    & FCN            & 25                                                               & 16                                                                                                                         & 0.919                                                         & 0.920                                                         & 0.920                                                          & 0.920                                                       \\
Pricing          & default                        & FCN            & 25                                                               & 16                                                                                                                         & 0.898                                                         & 0.903                                                         & 0.908                                                          & 0.903                                                       \\
Pricing          & default                        & XGB            & 25                                                               & 16                                                                                                                         & 0.897                                                         & 0.904                                                         & 0.896                                                          & 0.904                                                       \\
Pricing          & with\_feats                    & KNN            & 25                                                               & 16                                                                                                                         & 0.720                                                         & 0.755                                                         & 0.755                                                          & 0.755                                                       \\
Pricing          & default                        & KNN            & 25                                                               & 16                                                                                                                         & 0.699                                                         & 0.754                                                         & 0.707                                                          & 0.754                                                       \\
Pricing          & feat\_only                     & FCN            & 25                                                               & 16                                                                                                                         & 0.686                                                         & 0.700                                                         & 0.694                                                          & 0.700                                                       \\
Pricing          & feat\_only                     & XGB            & 25                                                               & 16                                                                                                                         & 0.684                                                         & 0.717                                                         & 0.688                                                          & 0.717                                                       \\
Pricing          & feat\_only                     & KNN            & 25                                                               & 16                                                                                                                         & 0.639                                                         & 0.673                                                         & 0.622                                                          & 0.673                                                       \\
Pricing          & with\_feats                    & XGB            & 50                                                               & 29                                                                                                                         & 0.894                                                         & 0.906                                                         & 0.893                                                          & 0.906                                                       \\
Pricing          & with\_feats                    & FCN            & 50                                                               & 29                                                                                                                         & 0.874                                                         & 0.880                                                         & 0.889                                                          & 0.880                                                       \\
Pricing          & default                        & XGB            & 50                                                               & 29                                                                                                                         & 0.873                                                         & 0.883                                                         & 0.876                                                          & 0.883                                                       \\
Pricing          & default                        & FCN            & 50                                                               & 29                                                                                                                         & 0.852                                                         & 0.857                                                         & 0.858                                                          & 0.857                                                       \\
Pricing          & with\_feats                    & KNN            & 50                                                               & 29                                                                                                                         & 0.701                                                         & 0.730                                                         & 0.698                                                          & 0.730                                                       \\
Pricing          & default                        & KNN            & 50                                                               & 29                                                                                                                         & 0.677                                                         & 0.697                                                         & 0.708                                                          & 0.697                                                       \\
Pricing          & feat\_only                     & XGB            & 50                                                               & 29                                                                                                                         & 0.673                                                         & 0.708                                                         & 0.709                                                          & 0.708                                                       \\
Pricing          & feat\_only                     & FCN            & 50                                                               & 29                                                                                                                         & 0.621                                                         & 0.643                                                         & 0.622                                                          & 0.643                                                       \\
Pricing          & feat\_only                     & KNN            & 50                                                               & 29                                                                                                                         & 0.556                                                         & 0.598                                                         & 0.544                                                          & 0.598                                                       \\
Pricing          & with\_feats                    & XGB            & 100                                                              & 43                                                                                                                         & 0.828                                                         & 0.842                                                         & 0.848                                                          & 0.842                                                       \\
Pricing          & default                        & XGB            & 100                                                              & 43                                                                                                                         & 0.821                                                         & 0.829                                                         & 0.834                                                          & 0.829                                                       \\
Pricing          & default                        & FCN            & 100                                                              & 43                                                                                                                         & 0.787                                                         & 0.793                                                         & 0.802                                                          & 0.793                                                       \\
Pricing          & with\_feats                    & FCN            & 100                                                              & 43                                                                                                                         & 0.752                                                         & 0.756                                                         & 0.763                                                          & 0.756                                                       \\
Pricing          & default                        & KNN            & 100                                                              & 43                                                                                                                         & 0.618                                                         & 0.652                                                         & 0.643                                                          & 0.652                                                       \\
Pricing          & feat\_only                     & XGB            & 100                                                              & 43                                                                                                                         & 0.606                                                         & 0.639                                                         & 0.614                                                          & 0.639                                                       \\
Pricing          & with\_feats                    & KNN            & 100                                                              & 43                                                                                                                         & 0.598                                                         & 0.625                                                         & 0.648                                                          & 0.625                                                       \\
Pricing          & feat\_only                     & FCN            & 100                                                              & 43                                                                                                                         & 0.565                                                         & 0.607                                                         & 0.564                                                          & 0.607                                                       \\
Pricing          & feat\_only                     & KNN            & 100                                                              & 43                                                                                                                         & 0.495                                                         & 0.526                                                         & 0.504                                                          & 0.526                                                       \\
Trace            & feat\_only                     & KNN            & 3                                                                & 3                                                                                                                          & 1.000                                                         & 1.000                                                         & 1.000                                                          & 1.000                                                       \\
Trace            & feat\_only                     & FCN            & 3                                                                & 3                                                                                                                          & 1.000                                                         & 1.000                                                         & 1.000                                                          & 1.000                                                       \\
Trace            & default                        & XGB            & 3                                                                & 3                                                                                                                          & 1.000                                                         & 1.000                                                         & 1.000                                                          & 1.000                                                       \\
Trace            & feat\_only                     & XGB            & 3                                                                & 3                                                                                                                          & 0.978                                                         & 0.978                                                         & 0.979                                                          & 0.978                                                       \\
Trace            & with\_feats                    & XGB            & 3                                                                & 3                                                                                                                          & 0.978                                                         & 0.978                                                         & 0.979                                                          & 0.978                                                       \\
Trace            & with\_feats                    & FCN            & 3                                                                & 3                                                                                                                          & 0.955                                                         & 0.956                                                         & 0.961                                                          & 0.956                                                       \\
Trace            & default                        & FCN            & 3                                                                & 3                                                                                                                          & 0.955                                                         & 0.956                                                         & 0.961                                                          & 0.956                                                       \\
Trace            & with\_feats                    & KNN            & 3                                                                & 3                                                                                                                          & 0.788                                                         & 0.800                                                         & 0.837                                                          & 0.800                                                       \\
Trace            & default                        & KNN            & 3                                                                & 3                                                                                                                          & 0.788                                                         & 0.800                                                         & 0.837                                                          & 0.800                                                       \\
Walmart          & with\_feats                    & XGB            & 10                                                               & 10                                                                                                                         & 0.905                                                         & 0.905                                                         & 0.906                                                          & 0.905                                                       \\
Walmart          & default                        & XGB            & 10                                                               & 10                                                                                                                         & 0.873                                                         & 0.872                                                         & 0.875                                                          & 0.872                                                       \\
Walmart          & default                        & KNN            & 10                                                               & 10                                                                                                                         & 0.856                                                         & 0.856                                                         & 0.864                                                          & 0.856                                                       \\
Walmart          & with\_feats                    & FCN            & 10                                                               & 10                                                                                                                         & 0.853                                                         & 0.853                                                         & 0.857                                                          & 0.853                                                       \\
Walmart          & with\_feats                    & KNN            & 10                                                               & 10                                                                                                                         & 0.846                                                         & 0.846                                                         & 0.849                                                          & 0.846                                                       \\
Walmart          & default                        & FCN            & 10                                                               & 10                                                                                                                         & 0.832                                                         & 0.831                                                         & 0.836                                                          & 0.831                                                       \\
Walmart          & feat\_only                     & XGB            & 10                                                               & 10                                                                                                                         & 0.797                                                         & 0.798                                                         & 0.798                                                          & 0.798                                                       \\
Walmart          & feat\_only                     & FCN            & 10                                                               & 10                                                                                                                         & 0.787                                                         & 0.788                                                         & 0.794                                                          & 0.788                                                       \\
Walmart          & feat\_only                     & KNN            & 10                                                               & 10                                                                                                                         & 0.716                                                         & 0.719                                                         & 0.719                                                          & 0.719                                                       \\
Walmart          & with\_feats                    & XGB            & 20                                                               & 20                                                                                                                         & 0.851                                                         & 0.852                                                         & 0.855                                                          & 0.852                                                       \\
Walmart          & default                        & XGB            & 20                                                               & 20                                                                                                                         & 0.850                                                         & 0.850                                                         & 0.853                                                          & 0.850                                                       \\
Walmart          & with\_feats                    & FCN            & 20                                                               & 20                                                                                                                         & 0.832                                                         & 0.833                                                         & 0.837                                                          & 0.833                                                       \\
Walmart          & default                        & FCN            & 20                                                               & 20                                                                                                                         & 0.823                                                         & 0.825                                                         & 0.826                                                          & 0.825                                                       \\
Walmart          & with\_feats                    & KNN            & 20                                                               & 20                                                                                                                         & 0.815                                                         & 0.817                                                         & 0.822                                                          & 0.817                                                       \\
Walmart          & default                        & KNN            & 20                                                               & 20                                                                                                                         & 0.802                                                         & 0.805                                                         & 0.808                                                          & 0.805                                                       \\
Walmart          & feat\_only                     & XGB            & 20                                                               & 20                                                                                                                         & 0.698                                                         & 0.703                                                         & 0.703                                                          & 0.703                                                       \\
Walmart          & feat\_only                     & FCN            & 20                                                               & 20                                                                                                                         & 0.680                                                         & 0.684                                                         & 0.703                                                          & 0.684                                                       \\
Walmart          & feat\_only                     & KNN            & 20                                                               & 20                                                                                                                         & 0.628                                                         & 0.637                                                         & 0.646                                                          & 0.637                                                       \\
Walmart          & with\_feats                    & XGB            & 40                                                               & 40                                                                                                                         & 0.796                                                         & 0.797                                                         & 0.809                                                          & 0.797                                                       \\
Walmart          & with\_feats                    & KNN            & 40                                                               & 40                                                                                                                         & 0.761                                                         & 0.768                                                         & 0.777                                                          & 0.768                                                       \\
Walmart          & default                        & KNN            & 40                                                               & 40                                                                                                                         & 0.759                                                         & 0.766                                                         & 0.778                                                          & 0.766                                                       \\
Walmart          & default                        & FCN            & 40                                                               & 40                                                                                                                         & 0.759                                                         & 0.762                                                         & 0.776                                                          & 0.762                                                       \\
Walmart          & with\_feats                    & FCN            & 40                                                               & 40                                                                                                                         & 0.729                                                         & 0.727                                                         & 0.757                                                          & 0.727                                                       \\
Walmart          & default                        & XGB            & 40                                                               & 40                                                                                                                         & 0.721                                                         & 0.723                                                         & 0.736                                                          & 0.723                                                       \\
Walmart          & feat\_only                     & XGB            & 40                                                               & 40                                                                                                                         & 0.606                                                         & 0.612                                                         & 0.616                                                          & 0.612                                                       \\
Walmart          & feat\_only                     & FCN            & 40                                                               & 40                                                                                                                         & 0.589                                                         & 0.607                                                         & 0.603                                                          & 0.607                                                       \\
Walmart          & feat\_only                     & KNN            & 40                                                               & 40                                                                                                                         & 0.477                                                         & 0.494                                                         & 0.486                                                          & 0.494                                                      
\end{tabular}
}

==> tables/R3/clustering_results.tex <==
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{lrrrrr}
\rowcolor[HTML]{B0B3B2} 
\textbf{Dataset}                & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{\# Clusters}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Silhouette Score}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Calinski-Harabasz Score}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Davies Bouldin Score}} & \multicolumn{1}{l}{\cellcolor[HTML]{B0B3B2}\textbf{Inertia}} \\
Electricity                     & 10                                                               & 0.144                                                                 & 59.64                                                                        & 1.733                                                                     & 1107                                                         \\
Electricity                     & 20                                                               & 0.104                                                                 & 40.42                                                                        & 1.524                                                                     & 854                                                          \\
Electricity                     & 30                                                               & 0.088                                                                 & 32.01                                                                        & 1.481                                                                     & 726                                                          \\
Electricity                     & 40                                                               & 0.075                                                                 & 26.84                                                                        & 1.537                                                                     & 646                                                          \\
Walmart                         & 10                                                               & 0.112                                                                 & 340.93                                                                       & 2.204                                                                     & 8096                                                         \\
Walmart                         & 20                                                               & 0.111                                                                 & 208.95                                                                       & 2.086                                                                     & 6978                                                         \\
Walmart                         & 30                                                               & 0.102                                                                 & 158.30                                                                       & 2.198                                                                     & 6364                                                         \\
Walmart                         & 40                                                               & 0.097                                                                 & 128.50                                                                       & 2.262                                                                     & 5998                                                         \\
Pricing                         & 25                                                               & -0.230                                                                & 3.65                                                                         & 3.104                                                                     & 6560                                                         \\
\cellcolor[HTML]{FFFFFF}Pricing & 50                                                               & -0.310                                                                & 3.79                                                                         & 2.692                                                                     & 6175                                                         \\
\cellcolor[HTML]{FFFFFF}Pricing & 75                                                               & -0.320                                                                & 3.43                                                                         & 2.542                                                                     & 5999                                                         \\
\cellcolor[HTML]{FFFFFF}Pricing & 100                                                              & -0.309                                                                & 3.27                                                                         & 2.424                                                                     & 5711                                                        
\end{tabular}
}
